HoneySat: A Network-based Satellite Honeypot Framework

Satellites are the backbone of several mission-critical services that enable our modern society to function, for example, GPS. For years, satellites were assumed to be secure because of their indecipherable architectures and the reliance on security by obscurity. However, technological advancements have made these assumptions obsolete, paving the way for potential attacks, and sparking interest in satellite security. Unfortunately, to this day, there is no efficient way to collect data on adversarial techniques for satellites, hurting the generation of security intelligence that can lead to the development of effective countermeasures. In this paper, we present HoneySat, the first high-interaction satellite honeypot framework, fully capable of convincingly simulating a real-world CubeSat, a type of Small Satellite (SmallSat). To provide evidence of HoneySat's effectiveness, we surveyed experienced SmallSat operators in charge of in-orbit satellites and deployed HoneySat over the Internet to entice adversaries. Our results show that 90% of satellite operators agreed that HoneySat provides a realistic and engaging simulation of a SmallSat mission. Additionally, HoneySat successfully deceived human adversaries in the wild and collected 22 real-world satellite-specific adversarial interactions. Finally, in a major demonstration of HoneySat's robustness, we collaborated with an aerospace company to perform a hardware-in-the-loop operation that resulted in HoneySat successfully communicating with an in-orbit, operational SmallSat mission.

==> figures/results/deception-experiments/camera-experiment.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.49\linewidth]{figures/results/deception-experiments/suchai-picture-example.jpeg}
    \includegraphics[width=0.49\linewidth]{figures/results/deception-experiments/camera-picture-example.jpg}
    \caption{Examples of Earth's surface picture provided by the SUCHAI-3 satellite and the \apiname. Credit: FCFM, University of Chile~\cite{uchileFacultyPhysical} and U.S. Geological Survey EarthExplorer Platform~\cite{usgsEarthExplorer}.}
    \label{fig:evaluation:camera-picture}
\end{figure}

==> figures/results/deception-experiments/comm-limit-result.tex <==
%\begin{figure}[t]
%    \centering
%    \includegraphics[width=8.5cm]{figures/results/deception-experiments/comm_limit.PNG}
%    \caption{\textbf{Provide realistic COM experiment GS log snippet.}}
%    \label{fig:evaluation:comm-limit}
%\end{figure}

\begin{comment}
\begin{figure}
\scriptsize
    \begin{verbatim}
[INFO ][1714319368][Executer] Running the command: com_ping...
OUT: S 10, D 1, Dp 1, Sp 41, Pr 2, Fl 0x00, Sz 10 VIA: ZMQHUB
INP: S 1, D 10, Dp 41, Sp 1, Pr 2, Fl 0x00, Sz 10 VIA: ZMQHUB
[RES  ][1714319369][cmdCOM] Ping to 1 took 1600
[INFO ][1714319369][Executer] Command result: 1
fp_set_cmd_dt 1 120 1 com_ping 1
[INFO ][1714319387][Executer] Running the command: fp_set_cmd_dt...
[INFO ][1714319387][Executer] Command result: 1
INFO ][1714319388][FlightPlan] Command: com_ping
[INFO ][1714319388][FlightPlan] Arguments: 1
[INFO ][1714319388][FlightPlan] Executions: 120
[INFO ][1714319388][FlightPlan] Period: 1
[INFO ][1714319388][Executer] Running the command: com_ping...
OUT: S 10, D 1, Dp 1, Sp 42, Pr 2, Fl 0x00, Sz 10 VIA: ZMQHUB
[INFO ][1714319389][FlightPlan] Command: com_ping
[INFO ][1714319389][FlightPlan] Arguments: 1
[INFO ][1714319389][FlightPlan] Executions: 119
[INFO ][1714319389][FlightPlan] Period: 1
[INFO ][1714319390][FlightPlan] Command: com_ping
[INFO ][1714319390][FlightPlan] Arguments: 1
[INFO ][1714319390][FlightPlan] Executions: 118
[INFO ][1714319390][FlightPlan] Period: 1
[INFO ][1714319391][FlightPlan] Command: com_ping
[INFO ][1714319391][FlightPlan] Arguments: 1
[INFO ][1714319391][FlightPlan] Executions: 117
[INFO ][1714319391][FlightPlan] Period: 1
[RES  ][1714319391][cmdCOM] Ping to 1 took -1
[INFO ][1714319391][Executer] Command result: 0
    \end{verbatim}
    \caption{\textbf{Snippets of \honeyname's GS log featuring a realistic COM.}}
    \label{fig:evaluation:comm-limit}
\end{figure}
\end{comment}


\lstset{style=TERMINAL_OUTPUT}

\begin{lstlisting}[float, caption=Snippet of \honeyname's MCS log featuring a realistic COM. The TC sequence shows pinging the satellite works (Command result:1) and then after the pass is over the ping fails (Command result:0)., label={listing:evaluation:comm-limit}]
[INFO ][1714319368][Executer] Running the command: com_ping...
OUT: S 10, D 1, Dp 1, Sp 41, Pr 2, Fl 0x00, Sz 10 VIA: ZMQHUB
INP: S 1, D 10, Dp 41, Sp 1, Pr 2, Fl 0x00, Sz 10 VIA: ZMQHUB
[RES  ][1714319369][cmdCOM] Ping to 1 took 1600
[INFO ][1714319369][Executer] Command result: 1
fp_set_cmd_dt 1 120 1 com_ping 1
[INFO ][1714319387][Executer] Running the command: fp_set_cmd_dt...
[INFO ][1714319387][Executer] Command result: 1
[INFO ][1714319388][FlightPlan] Command: com_ping
[INFO ][1714319388][FlightPlan] Arguments: 1
[INFO ][1714319388][FlightPlan] Executions: 120
[INFO ][1714319388][FlightPlan] Period: 1
[INFO ][1714319388][Executer] Running the command: com_ping...
OUT: S 10, D 1, Dp 1, Sp 42, Pr 2, Fl 0x00, Sz 10 VIA: ZMQHUB
[INFO ][1714319389][FlightPlan] Command: com_ping
[INFO ][1714319389][FlightPlan] Arguments: 1
[INFO ][1714319391][FlightPlan] Executions: 117
[INFO ][1714319391][FlightPlan] Period: 1
\hl{[RES  ][1714319391][cmdCOM] Ping to 1 took -1}
[INFO ][1714319391][Executer] Command result: 0
\end{lstlisting}

\lstset{style=TC_commands}


==> figures/results/deception-experiments/eps-get-results.tex <==
\begin{comment}
\begin{figure}
    \begin{verbatim}
        Running the command: tm_get_last...
        sat_index: 0
        timestamp: 1714061113
        vbatt: 8027
        temp_eps: 24
        temp_bat: 24
    \end{verbatim}
    \caption{\textbf{EPS TM experiment \apiname log data.}}
    \label{fig:evaluation:eps}
\end{figure}
\end{comment}


\lstset{style=TERMINAL_OUTPUT}

\begin{lstlisting}[float, caption=\apiname log output for EPS TM experiment., label={listing:evaluation:eps}]
Running the command: tm_get_last...
sat_index: 0
timestamp: 1714061113
vbatt: 8027
temp_eps: 24
temp_bat: 24
\end{lstlisting}


%\lstset{style=TC_commands}
            

%Received request: b'\x02\x00'
%EPS HK: VBat=8027, CurrIn=0,
%CurrOut=74, Temp=24
%Sending reply: b'[\x1f\x00\x00
%\x00\x00\x00\x00J\x00\x00\x00
%\x18\x00\x00\x00'


